Sounding Bodies: Modeling 3D Spatial Sound of Humans Using Body Pose and Audio

While 3D human body modeling has received much attention in computer vision, modeling the acoustic equivalent, i.e. modeling 3D spatial audio produced by body motion and speech, has fallen short in the community. To close this gap, we present a model that can generate accurate 3D spatial audio for full human bodies. The system consumes, as input, audio signals from headset microphones and body pose, and produces, as output, a 3D sound field surrounding the transmitter's body, from which spatial audio can be rendered at any arbitrary position in the 3D space. We collect a first-of-its-kind multimodal dataset of human bodies, recorded with multiple cameras and a spherical array of 345 microphones. In an empirical evaluation, we demonstrate that our model can produce accurate body-induced sound fields when trained with a suitable loss. Dataset and code are available online.

==> sections/new_task.tex <==
% !TEX root = ../main.tex

\section{Pose-Guided 3D Spatial Audio Generation}

\ar{TODO: high-level overview - clarify input/output and focus on challenges}

\subsection{Problem Formulation}
\label{sec:problem_formulation}

Let $ \mathbf{a}_{1:T} = (a_1, \dots, a_T) $ be an audio signal of length $ T $ captured by the head-mounted microphones, where $ T $ indicates the number of samples, and each $ a_t \in \mathbb{R}^{C_{\text{in}}} $ represents the value of the waveform at time $ t $ for each of the $ C_\text{in} $ input channels.
Let further $ \mathbf{p}_{1:S} = (p_1, \dots, p_S) $ be the temporal stream of body pose, where each $ p_s \in \mathbb{R}^{J \times 3} $ represents the 3D coordinates of each of the $ J $ body joints at the visual frame $ s $.
Note that audio signals $ \mathbf{a}_{1:T} $ and pose data $ \mathbf{p}_{1:S} $ are of the same duration, but sampled at a different rate.
In this work, audio is sampled at 48kHz and pose at 30 fps, so there is one new pose frame for every 1,600 audio samples.

Ideally, we would like to learn a transfer function $ \mathcal{T} $ that maps from the head-mounted microphone signals and body pose directly to the audio signal $ \mathbf{s}_{1:T} $ at any arbitrary coordinate $ (x,y,z) $ in the 3D space,
\begin{align}
    \mathbf{s}_{1:T}(x,y,z) = \mathcal{T}\big(x, y, z, \mathbf{a}_{1:T}, \mathbf{p}_{1:S}\big).
\end{align}
However, it is in practice impossible to densely populate a 3D space with microphones and record the necessary training data.
Instead, our capture stage is a spherical microphone array and data can only be measured on the surface of this sphere, \ie at microphone positions defined by their polar coordinates $ (\theta, \phi, r) $.
Since the radius $ r $ is the same for every point on the sphere, a microphone position is uniquely defined by its azimuth $ \theta $ and elevation $ \phi $.
Leveraging the recordings of the microphones on the sphere as supervision, we model a transfer function
\begin{align}
    \mathbf{s}_{1:T}(\theta_i, \phi_i) = \mathcal{T}\big(\theta_i, \phi_i, \mathbf{a}_{1:T}, \mathbf{p}_{1:S}\big)
\end{align}
that maps from input audio $ \mathbf{a}_{1:T} $ and body pose $ \mathbf{p}_{1:S} $ to the signal recorded by microphone $ i $ which is located at $ (\theta_i, \phi_i) $ on the sphere.

In order to render sound at an arbitrary position $ (x,y,z) $ in 3D space, we predict $ \mathbf{s}_{1:T}(\theta, \phi) $ for all microphone positions $ (\theta_i, \phi_i) $ on the sphere, and encode them into harmonic sound field coefficients~\misscite, from which the signal $ \mathbf{s}_{1:T} $ can then be rendered at any arbitrary spatial position $ (x,y,z) $, see Section~\ref{subsec:rendering} for details.
In the following sections, we describe the design of the network modeling the transfer function $ \mathcal{T} $ and its training algorithm.


\subsection{Network Architecture}
\label{sec:network_architecture}

\mathbf{Audio Encoder.}

\mathbf{Pose Encoder.}

\mathbf{Audio Decoder.}



% Our goal is to learn a transfer function $ \mathcal{T} $ that maps from head-mounted microphones and body pose onto the signal that would be recorded at position $ (\theta, \phi) $ on the spherical microphone array surrounding the participant at training data capture time,
% \begin{align}
%     \mathbf{s}_{1:T}^{(i)} = \mathcal{T}(\mathbf{a}_{1:T}, \mathbf{p}_{1:S} | \mathbf{m}_i)
% \end{align}

% We define a position on the spherical microphone array by its azimuth $ \theta $ and elevation $ \phi $, so that microphone $ i $ is uniquely identified by its position $ (\theta_i, \phi_i) $.
% Then, the sound recorded of microphone $ i $ is $ \mathbf{s}_{1:T}(\theta_i, \phi_i) $.


% We further denote the signal recorded by the microphones on the spherical array as $ \mathbf{s}_{1:T}^{(i)} = (s_1^{(i)}, \dots, s_T^{(i)} ) $, where $ s_t^{(i)} \in \mathbb{R} $ and $ i $ is the $i$-th microphone at position $ \mathbf{m}_i = (x_i, y_i, z_i) $ in the array.

% Our goal is to learn a transfer function $ \mathcal{T} $ that maps from head-mounted microphones and body pose onto the signal that a microphone at position $ \mathbf{m}_i $ in the spherical array would record,
% \begin{align}
%     \mathbf{s}_{1:T}^{(i)} = \mathcal{T}(\mathbf{a}_{1:T}, \mathbf{p}_{1:S} | \mathbf{m}_i)
% \end{align}


% As mentioned in Sec.~\ref{sec:intro}, 3D spatial audio, along with the photorealistic renderings, is the prerequisite of high-fidelity 3D avatars.
% Actually, spatial audio is inherently affected by the corresponding human body pose.
% In this paper, we are the first to explore this novel problem and hence propose a new task, \textbf{pose-guided 3D spatial audio generation}, \ie, generating spatial audio of any 3D position based on human pose in order to recover the whole sound field.

% In a given environment $\cE$, a single person is talking or making body sounds, including clapping, snapping, or tapping his thigh.
% Assuming there are $K$ microphones mounted on the participant's head responsible for recording the sounds,
% given the $K$-channel recorded sound $\va_k, k=1,2, ..., K$, the microphone position $\vm_k = (x_k, y_k, z_k), k=1,2, ..., K$, as well as the corresponding 3D human pose $\mP$,
% the goal of this task is to faithfully generate the audio $\va_i$ of the target mic located in $\vm_i = (x_i, y_i, z_i)$ in the near field.
% The whole pipeline is illustrated in Fig.~\ref{fig:teaser}.
% %
% Therefore, our goal is to learn a transfer function $\cT(\cdot)$ defined as:
% \begin{align}
%     \va_i = \cT \left( \va_{1,...,K}, \vm_{1,...,K}, \mP, \vm_i \big| \cE \right).
%     \label{eq:orig_formula}
% \end{align}
% Once the audio $\va_i$ at any 3D coordinate can be generated, we are able to infer the whole sound field accordingly.
% However, this task is extremely challenging since the transfer function $\cT$ is not a linear time-invariant system and is significantly affected by several acoustic effects, like room reverberations and complex diffraction while sound travels around the human torso.

% To simplify this problem, we capture all the data in an anechoic chamber, thus getting rid of the room reverberations.
% The OpenPose~\cite{cao2017realtime} format of $25$ keypoints is used to stand for the 3D human pose $\mP$. \dm{We actually use only 19 of these 25 keypoints (the 3 foot keypoints for both legs are not used) although I'm sure nothing would happen if we were to include those as well}
% %Besides, the headset microphone positions $\vx_{1,...,N}$ can be represented with keypoints of eyes plus a fixed offset and hence be omitted for simplification.
% %For $N$ recorded sounds, we select only one audio from the microphone located in the middle of the VR headset~\missref.
% Besides, $K$ recording microphones are all mounted on the head and their positions $\vm_k$ can be represented with a fixed linear combination of keypoints on the head $\mP_\text{H}$: $\vm_k = FC(\mP_\text{H})$.
% % where $\mP_\text{H}$ is dubbed as head pose in the following.
% Hence, we omit $\vm_k$ for simplification and the transfer function $\cT$ in Eq.~\ref{eq:orig_formula} now becomes
% \begin{align}
%     \va_i = \cT \left( \va_{1,...,K}, \mP, \vm_i \right).
%     \label{eq:formula}
% \end{align}
% It's noteworthy that complex diffraction is still an inevitable problem despite such simplifications and will significantly modify the emitted sound.
% Thus, the sound propagation here can't be naively modeled as the free-field propagation, and the transfer function $\cT$ cannot be regarded as a simple time shift.


